Sparsifying the Operators of Fast Matrix Multiplication Algorithms

Fast matrix multiplication algorithms may be useful, provided that their running time is good in practice. Particularly, the leading coefficient of their arithmetic complexity needs to be small. Many sub-cubic algorithms have large leading coefficients, rendering them impractical. Karstadt and Schwartz (SPAA'17, JACM'20) demonstrated how to reduce these coefficients by sparsifying an algorithm's bilinear operator. Unfortunately, the problem of finding optimal sparsifications is NP-Hard. We obtain three new methods to this end, and apply them to existing fast matrix multiplication algorithms, thus improving their leading coefficients. These methods have an exponential worst case running time, but run fast in practice and improve the performance of many fast matrix multiplication algorithms. Two of the methods are guaranteed to produce leading coefficients that, under some assumptions, are optimal.

==> fastbasis/fastbasis.tex <==
\section{Alternative Basis Matrix Multiplication}\label{sec:Alternative-Basis-Strassen-like}

Fast matrix multiplication algorithms are bilinear computations. The number of operations performed in the linear phases of such algorithms (the application of its encoding/decoding matrices $\encdec{U}{V}{W}$ in the case of matrix multiplication, see Definition \ref{def:encdec}) depends on basis of representation. In this section, we detail how alternative basis algorithms work and address the effects of using alternative bases on arithmetic complexity and IO-complexity.


\begin{definition}
Let $R$ be a ring and let $\bmapss$ be automorphisms of $R^{n\cdot m} , \, R^{m\cdot k}, \, R^{n\cdot k}$ (respectively).
We denote a Strassen-like algorithm which takes $\phi \left(A\right),\,\psi\left(B\right)$
as inputs and outputs $\upsilon \left(A\cdot B\right)$ using $t$ multiplications. $ \strassaltdef{n}{m}{k}{t} $ \\
If $n=m=k$ and $\phi=\psi=\upsilon$ we use the notation $\squarestrass{n}{t}_{\phi}$-algorithm. This notation
extends the $\strass{n}{m}{k}{t}$-algorithm notation as latter applies when the three basis transformations are the identity map.
\end{definition}

Given a recursive-bilinear, $\strassaltdef{n}{m}{k}{t}$-algorithm, {\em ALG}, alternative basis matrix multiplication works as follows:

\begin{algorithm}[h]
	\begin{algorithmic}[1]
	\Require{$A\in R^{n\times m}$, $B^{m\times k}$}
	\Ensure{$n\times k$ matrix $C = A\cdot B$}
    	\Function{$ABS$}{$A,B$}
			\State $\tilde{A} = \phi (A)$ \Comment{$R^{n\times m}$ basis transformation}
			\State $\tilde{B} = \psi (B)$ \Comment{$R^{m\times k}$ basis transformation}
			\State $\tilde{C} = ALG (\tilde{A},\tilde{B})$ \Comment{$\strassalt{n}{m}{k}{t}{\phi}{\psi}{\upsilon}$-algorithm }
			\State $C = \upsilon^{-1}(\tilde{C})$ \Comment{$R^{n\times k}$ basis transformation}    
		\EndFunction
\State \Return{$C$}
	\end{algorithmic}
	\caption{\label{alg:ABS}Alternative Basis Matrix Multiplication Algorithm}
\end{algorithm}

\begin{lemma}\cite{}\label{cor:alt to mul}Let $R$ be a ring, and let $\bmapss$ be automorphisms of $R^{n\cdot m},\,R^{m\cdot k},\,R^{n\cdot k}$ (respectively). $\encdec{U}{V}{W} $
are encoding/decoding matrices of an $\strassaltdef{n}{m}{k}{t}$-algorithm if and only if $\encdec{U\phi}{V\psi}{W\upsilon^{-T}}$ are encoding/decoding matrices of an $\strass{n}{m}{k}{t}$-algorithm
\end{lemma}

\subsection{Fast basis transformation\label{subsec:basis}}

\begin{definition}
\label{def:rec-transform} Let $R$ be a ring and let 
$\psi_{1}:R^{n_{0}\times m_{0}}\to R^{n_{0}\times m_{0}}$
be a linear map. We recursively define a linear map $\psi_{k+1}:R^{n\times m}\to R^{n\times m}$
(where $n=n_{0}^{\ell _1}, \, m=m_{0}^{\ell _2}$ for some $\ell _1, \, \ell _2\leq k+1$) by $\left(\psi_{k+1}\left(A\right)\right)_{i,j}=\psi_{k}\left(\psi_{1}\left(A\right)\right)_{i,j} $, where $A_{i,j}$ are sub-matrices of size $\frac{n}{n_{0}}\times \frac{m}{m_{0}}$ .
\end{definition}

Note that $\psi_{k+1}$ is a linear map. For convenience, we omit the subscript of $\psi$ when obvious from context.
\begin{lemma}
\label{lem:order-switch-basis}Let $R$ be a ring, let $\psi_{1}:R^{n_{0}\times m_{0}}\to R^{n_{0}\times m_{0}}$
be a linear map, and let $A\in R^{n\times m}$ (where $n=n_{0}^{k+1}, \, m=m_{0}^{k+1}$).
Let us define $\tilde{A}$ by $\left(\tilde{A}\right)_{i,j}=\psi_{k}\left(A_{i,j}\right)$. Then $ \psi_{1}\left(\tilde{A}\right)=\psi_{k+1}\left(A\right) $.
\begin{proof}
$\psi_{1}$ is a linear map. Hence, $\forall i,\,j\in\left[n\right]\:\left(\psi_{1}\left(A\right)\right)_{i,j}=\sum\limits _{\ell_{1},\ell_{2}\in\left[n\right]}x_{k_{1},k_{2}}^{\left(i,j\right)}\cdot A_{i,j}$
where $A$ is treated as an $\frac{n}{n_{0}}\times\frac{n}{n_{0}}$
block matrix and $x_{\ell_{1},\ell_{2}}^{\left(i,j\right)}\in R$
are scalars.

By Definition \ref{def:rec-transform}
\begin{align*}
\left(\psi_{k+1}\left(A\right)\right)_{i,j} & =\psi_{k}\left(\psi_{1}\left(A\right)\right)_{i,j}\\
 & =\psi_{k}\left(\sum\limits _{\ell_{1},\ell_{2}\in\left[n\right]}x_{\ell_{1},\ell_{2}}^{\left(i,j\right)}\cdot A_{\ell_{1},\ell_{2}}\right)\\
\text{By linearity of }\psi_{k}\\
 & =\sum\limits _{\ell_{1},\ell_{2}\in\left[n\right]}x_{\ell_{1},\ell_{2}}^{\left(i,j\right)}\psi_{k}\left(A_{\ell_{1},\ell_{2}}\right) =\left(\psi_{1}\left(\tilde{A}\right)\right)_{i,j}
\end{align*} 
%See Appendix \ref{subsec:Basis-proofs}
\end{proof}
\end{lemma}

\begin{lemma}
\label{lem:basis-invert}Let $R$ be a ring, let $\psi_{1}:R^{n_{0}\times m_{0}}\to R^{n_{0}\times m_{0}}$
be an invertible linear map, and let $\psi_{k+1}$ as defined above.
$\psi_{k+1}$ is invertible and its inverse is $\left(\psi_{k+1}^{-1}\left(A\right)\right)_{i,j}=\psi_{k}^{-1}\left(\psi_{1}^{-1}\left(A\right)\right)_{i,j}$.
\begin{proof}
Let us define $\tilde{A}$ by $\left(\tilde{A}\right)_{i,j}=\psi_{k}\left(A_{i,j}\right)$
and define $\psi_{k+1}^{-1}$ by $\left(\psi_{k+1}^{-1}\left(A\right)\right)_{i,j}=\psi_{k}^{-1}\left(\psi_{1}^{-1}\left(A\right)\right)_{i,j}$.
Then:

\begin{align*}
\left(\psi_{k+1}^{-1}\left(\psi_{k+1}\left(A\right)\right)\right)_{i,j} & =
\psi_{k}^{-1}\left(\psi_{1}^{-1}\left(\psi_{k+1}\left(A\right)\right)\right)_{i,j}\\
\text{By Lemma \ref{lem:order-switch-basis}}\\
 & =\psi_{k}^{-1}\left(\psi_{1}^{-1}\left(\psi_{1}\left(\tilde{A}\right)\right)\right)_{i,j}=\psi_{k}^{-1}\left(\tilde{A}\right)_{i,j}\\
\text{By definition of }\tilde{A}\\
 & =\psi_{k}^{-1}\left(\psi_{k}\left(A\right)_{i,j}\right)=A_{i,j}
\end{align*}
%In appendix \ref{subsec:Basis-proofs}
\end{proof}
\end{lemma}

We next analyze the arithmetic complexity and IO-complexity of fast basis transformations. For convenience and readability, we presented here the square case only. The analysis for rectangular matrices is similar.

\begin{lemma}
\label{lem:basis runtime-1}Let $R$ be a ring, let $\psi_{1}:R^{n_{0}\times n_{0}}\to R^{n_{0}\times n_{0}}$
be a linear map, and let $A\in R^{n\times n}$ where $n=n_{0}^{k}$.
The arithmetic complexity of computing $\psi$ is 
\[
F_{\psi}\left(n\right)=\frac{q}{n_{0}^{2}}n^{2}\log_{n_{0}}n
\]
where $q$ is the number of linear operations performed by $\psi_{1}$.
\begin{proof}
By straightforward expansion of the recurrence relation. See Appendix \ref{subsec:Basis-proofs}.
\end{proof}
\end{lemma}
%
\begin{lemma}
\label{lem:basis bw-1}Let $R$ be a ring and let $\psi_{1}:R^{n_{0}\times n_{0}}\to R^{n_{0}\times n_{0}}$
be an invertible linear map, and let $A\in R^{n\times n}$ where $n=n_{0}^{k}$.
The IO-complexity of computing $\psi$ is 
\[
IO_{\psi}\left(n,M\right)\leq\frac{3q}{n_{0}^{2}}n^{2}\log_{n_{0}}\left(\sqrt{2}\frac{n}{\sqrt{M}}\right)+2M
\]
where $q$ is the number of linear operations performed by $\psi_{1}$.
\begin{proof}
By straightforward expansion of the recurrence relation. See Appendix \ref{subsec:Basis-proofs}.
\end{proof}
\end{lemma}

\subsection{Computing matrix multiplication in alternative basis\label{subsec:bilinear}}
\begin{claim}
Let $\phi_{1},\psi_{1},\upsilon_{1}$ be automorphisms of $R^{n_{0}\times m_{0}}, R^{m_{0}\times k_{0}}, $ $R^{n_{0}\times k_{0}}$ (respectively), and let {\em ALG} be an $\strassalt{n_{0}}{m_{0}}{k_{0}}{t}{\phi_1}{\psi_1}{\upsilon_1}$ -algorithm. For any $A\in R^{n\times m}$, $\,B\in R^{m\times k}$, where $n=n_{0}^{\ell},\,m=m_{0}^{\ell},\,k=k_{0}^{\ell}$. Then 
\[
ALG\left(\phi_{\ell}\left(A\right),\psi_{\ell}\left(B\right)\right) = \upsilon_{\ell}\left(A\cdot B\right)
\]

\begin{proof}
Denote $\tilde{C} = ALG\left(\phi_{\ell+1}\left(A\right),\psi_{\ell+1}\left(B\right)\right)$ and the encoding/decoding matrices of {\em ALG} by $\encdec{U}{V}{W}$. We prove by induction on $\ell$ that $\tilde{C} = \upsilon_{\ell}\left(A\cdot B\right)$.
For $r\in\left[t\right]$, denote

\begin{align*}
S_{r} &=\sum\limits _{i\in \left[n_{0}\right],j\in\left[m_{0}\right]}U_{r,\left(i,j\right)}\left(\phi_{1}\left(A\right)\right)_{i,j}\\
T_{r}&=\sum\limits _{i\in \left[m_{0}\right],j\in\left[k_{0}\right]}V_{r,\left(i,j\right)}\left(\psi_{1}\left(B\right)\right)_{i,j}
\end{align*}

The base case, $\ell = 1$, holds by Lemma \ref{lem:mul to alternate} as {\em ALG} is an $\strassalt{n_{0}}{m_{0}}{k_{0}}{t}{\phi_1}{\psi_1}{\upsilon_1}$-algorithm. Note that this means that for any $i\in\left[n_{0}\right], \, j\in\left[ k_{0}\right]$
\begin{align*}
	\left(\upsilon_{1}\left(A B\right)\right)_{i,j}& = \left(W^{T}\left(\left(U\cdot\phi_{1}\left(A\right)\right)\odot \left( V\cdot \psi_{1} \left(B\right)\right)\right)\right)_{i,j} \\
	&=\sum_{r\in\left[t\right]}W_{r,\left(i,j\right)}\left(S_{r}\cdot T_{r}\right)
\end{align*}

Next, we assume the claim holds for $\ell \in \mathbb{N}$ and show for $\ell + 1$. 
Given input $\tilde{A}=\phi_{\ell+1}\left(A\right),\,\tilde{B}=\psi_{\ell+1}\left(B\right)$, {\em ALG} performs $t$ multiplications $P_{1},\ldots,P_{t}$. For each multiplication $P_{r}$, its left hand side multiplicand is of the form
\[
L_{r} =\sum\limits _{i\in \left[n_{0}\right],j\in\left[m_{0}\right]}U_{r,\left(i,j\right)}\tilde{A}_{i,j}
\]
By definition, $\left(\phi_{\ell+1}\left(A\right)\right)_{i,j}=\phi_{\ell}\left(\phi_{1}\left(A\right)\right)_{i,j}$. Hence,
\[
=\sum\limits _{i\in \left[n_{0}\right],j\in\left[m_{0}\right]}U_{r,\left(i,j\right)}\left(\phi_{\ell}\left(\phi_{1}\left(A\right)\right)_{i,j}\right)
\]
From linearity of $\phi_{\ell}$
\begin{align*}
    &=\phi_{\ell}\left(\sum\limits _{i\in \left[n_{0}\right],j\in\left[m_{0}\right]}U_{r,\left(i,j\right)}\left(\phi_{1}			\left(A\right)\right)_{i,j}\right) \\
	&= \phi_{\ell}\left(S_{r}\right)
\end{align*}
And similarly, the right hand multiplication $R_{r}$ is of the form
\[
R_{r} = \psi_{\ell}\left(T_{r}\right)
\]
Note that for any $r \in \left[t\right]$, $S_{r},\, T_{r}$ are $n_{0}^{\ell}\times m_{0}^{\ell}$ and $m_{0}^{\ell}\times k_{0}^{\ell}$ matrices, respectively.
Hence, by the induction hypothesis,
\[
P_{r} = ALG\left(\phi_{\ell}\left(S_{r}\right),\psi_{\ell}\left(T_{r}\right)\right)=\upsilon_{\ell}\left(S_{r}\cdot T_{r}\right)
\]
Each entry in the output $\tilde{C}$ is of the form:
\begin{align*}
	\tilde{C}_{i,j} & =\sum_{r\in\left[t\right]}W_{r,\left(i,j\right)}P_{r} \\
	& =\sum_{r\in\left[t\right]}W_{r,\left(i,j\right)}\upsilon_{\ell}\left(S_{r}\cdot T_{r}\right)
\end{align*}
By linearity of $\upsilon_{\ell}$
\[
=\upsilon_{\ell}\left(\sum_{r\in\left[t\right]}W_{r,\left(i,j\right)}\left(S_{r}\cdot T_{r}\right)\right)
\]
And, as noted in the base case:
\[
\left(\upsilon_{1}\left(A\cdot B\right)\right)_{i,j} = \left(\sum_{r\in\left[t\right]}W_{r,\left(i,j\right)}\left(S_{r}\cdot T_{r}\right)\right)_{\left(i,j\right)}
\]
Hence,
\[
\tilde{C}_{i,j} = \upsilon_{\ell} \left(\upsilon_{1}\left(A\cdot B\right)\right)_{i,j}
\]
Therefore, by Definition \ref{def:rec-transform}, $\tilde{C} = \upsilon_{\ell+1}\left(A\cdot B\right)$
\end{proof}
\end{claim}

\begin{lemma}
\label{lem:RABS-flops}Let {\em ALG} be an $\squarestrassaltdef{n_0}{t}$-algorithm which performs $q$ linear operations at its base case.
The arithmetic complexity of {\em ALG} is
\[
 F_{ALG}\left(n\right)=\left(1+\frac{q}{t-n_{0}^{2}}\right)n^{\omega_{0}}-\left(\frac{q}{t-n_{0}^{2}}\right)n^{2}
\]
where $\omega_{0}=\log_{n_{0}}t$.
\begin{proof}
By straightforward expansion of the recurrence relation. See Appendix \ref{subsec:Bilinear-proofs}
\end{proof}
\end{lemma}

\begin{lemma}
\label{lem:bilinear bw-1}Let {\em ALG} be an $\squarestrassaltdef{n_{0}}{t}$-algorithm which performs $q$ linear operations at its base case.
The IO-complexity of {\em ALG} is 
\begin{align*}
IO_{ALG}\left(n,M\right) \leq & \left(\frac{q}{t-n_{0}^{2}}\right)\left(M\left(\sqrt{3}\cdot\frac{n}{\sqrt{M}}\right)^{\omega_{0}}-3n^{2}\right)+3M
\end{align*}
where $\omega_{0}=\log_{n_{0}}t$.
\begin{proof}
By straightforward expansion of the recurrence relation. See Appendix \ref{subsec:Bilinear-proofs}
\end{proof}
\end{lemma}

\begin{corollary}\label{cor:absflops}
If {\em ABS} (Algorithm \ref{alg:ABS}) performs $q$ linear operations at the base case, then its arithmetic complexity is
\begin{align*}
F_{ABS}\left(n\right)=&\left(1+\frac{q}{t-n_{0}^{2}}\right)n^{\omega_{0}}-\left(\frac{q}{t-n_{0}^{2}}\right)n^{2} + O\left(n^2\log n\right)
\end{align*}
where $\omega_{0}=\log_{n_{0}}t$.

	\begin{proof}
	The number of flops performed by the algorithm is the sum of: (1) the number of flops performed by the basis transformations (denoted $\bmapss$) and (2) the number of flops performed by the recursive bilinear algorithms {\em ALG}.
	\[
		F_{ABS}\left(n\right) = F_{ALG}\left(n\right) + F_{\phi}\left(n\right)+ F_{\psi}\left(n\right) + F_{\upsilon}\left(n\right)
	\]
By Lemma \ref{lem:basis runtime-1} and Lemma \ref{lem:RABS-flops}
\begin{align*}
F_{ABS}\left(n\right)= & \left(1+\frac{q}{t-n_{0}^{2}}\right)n^{\omega_{0}}-\left(\frac{q}{t-n_{0}^{2}}\right)n^{2} + O\left(n^2\log n\right)
\end{align*}
	\end{proof}
\end{corollary}
%
\begin{corollary}\label{cor:absbw}
If {\em ABS} (Algorithm \ref{alg:ABS}) performs $q$ linear operations at the base case, then its IO-complexity is
%Let $\bmapss:R^{n_{0}\times n_{0}}\to R^{n_{0}\times n_{0}}$ be invertible linear maps, and let {\em ALG} be an \\ $\squarestrassaltdef{n_{0}}{t}$-algorithm which performs $q$ linear operations at the base case.
%The IO-complexity of {\em ABS} (Algorithm \ref{alg:ABS}) is
	\begin{align*}
	  IO_{ALG}\left(n,M\right) \leq & \left(\frac{3q}{t-n_{0}^{2}}\right)\left(M\left(\frac{\sqrt{3}\cdot n}{\sqrt{M}}\right)^{\omega_{0}}-n^{2}\right) + \\
	  & +3M + O\left(n^2\log \frac{n}{\sqrt{M}} \right)	
	\end{align*}
where $\omega_0 = \log_{n_0} t$.

	\begin{proof}
	The IO-complexity is the sum of: (1) the IO-complexity of the basis transformations (denoted $\bmapss$) and (2) the IO-complexity of the recursive bilinear algorithms {\em ALG}.
\begin{align*}
		IO_{ABS}\left(n,M\right) =&  IO_{ALG}\left(n,M\right) + IO_{\phi}\left(n,M\right)+\\
		&+ IO_{\psi}\left(n,M\right) + IO_{\upsilon}\left(n,M\right)
\end{align*}
By Lemma \ref{lem:basis bw-1} and Lemma \ref{lem:bilinear bw-1}

	\begin{align*}
	  IO_{ABS}\left(n,M\right) \leq & \left(\frac{3q}{t-n_{0}^{2}}\right)\left(M\left(\frac{\sqrt{3}\cdot n}{\sqrt{M}}\right)^{\omega_{0}}-n^{2}\right) + \\
	  & +3M + O\left(n^2\log \frac{n}{\sqrt{M}} \right)	
	\end{align*}
	\end{proof}

\end{corollary}

==> fastbasis/optstrass.tex <==
\subsection{Optimal $\squarestrass{2}{7}$-algorithm} \label{subsec:optstrass}

We now present a basis transformation $\psi_{opt}:R^{4}\to R^{4}$ and an $\squarestrass{2}{7}_{\psi}$-algorithm which performs only 12 linear operations.

\begin{notation} \label{notation:optbase} Let, $\psi_{opt}$ refer to the following transformation:
\[
\psi_{opt}=\begin{pmatrix*}[r] 1 & 0 & 0 & 0\\
0 & 1 & -1 & 1\\
0 & 0 & -1 & 1\\
0 & 1 & 0 & 1
\end{pmatrix*}\quad \psi_{opt}^{-1}=\begin{pmatrix*}[r] 1 & 0 & 0 & 0\\
0 & 1 & -1 & 0\\
0 & -1 & 0 & 1\\
0 & -1 & 1 & 1
\end{pmatrix*}
\]
\end{notation}

For convenience, when applying $\psi$ to matrices, we omit the
vectorization and refer to it as $\psi:R^{2\times 2}\to R^{2\times 2}$:
\begin{align*}
\psi_{opt}\left(A\right) & =\psi_{1}\begin{pmatrix*}[r] A_{1,1} & A_{1,2}\\
A_{2,1} & A_{2,2}
\end{pmatrix*} =\begin{pmatrix*} A_{1,1} & A_{1,2}-A_{2,1}+A_{2,2}\\
A_{21}-A_{2,2} & A_{1,2}+A_{2,2}
\end{pmatrix*}
\end{align*}
Where $A_{i,j}$ can be ring elements or sub-matrices. $\psi_{opt}^{-1}$ is defined analogously. Both $\psi_{opt}$ and $\psi_{opt}^{-1}$ extend recursively as in Definition \ref{def:rec-transform}.

\begin{figure}[th]

\[
\encdec{U_{opt}}{V_{opt}}{W_{opt}} =
\]
%\centering
\[ \left \langle
\begin{pmatrix*}[r] 0 & 0 & 0 & 1\\
0 & 0 & 1 & 0\\
0 & 1 & 0 & 0\\
1 & 0 & 0 & 0\\
0 & 1 & -1 & 0\\
-1 & 1 & 0 & 0\\
0 & -1 & 0 & 1
\end{pmatrix*},\,
\begin{pmatrix*}[r] 0 & 0 & 0 & 1\\
0 & 0 & 1 & 0\\
0 & 1 & 0 & 0\\
1 & 0 & 0 & 0\\
0 & -1 & 0 & 1\\
0 & 1 & -1 & 0\\
-1 & 1 & 0 & 0
\end{pmatrix*} ,\, 
\begin{pmatrix*}[r] 0 & 0 & 0 & 1\\
0 & 0 & 1 & 0\\
0 & 1 & 0 & 0\\
1 & 0 & 0 & 0\\
1 & 1 & 0 & 0\\
0 & -1 & 0 & -1\\
0 & 1 & 1 & 0
\end{pmatrix*}
\right \rangle
\]

\caption{$\encdec{U}{V}{W}$ are the encoding/decoding matrices of our $\squarestrass{2}{7}_{\psi}$-algorithm which performs 12 linear operations}
\label{fig:optstrass}
\end{figure}

\begin{claim}
\label{lem:RABS BASE}$\encdec{U_{opt}}{V_{opt}}{W_{opt}}$
are encoding/decoding matrices of an $\squarestrass{2}{7}_{\psi}$-algorithm.
\begin{proof}
Observe that 
\[
\encdec{U_{opt}\cdot\psi_{opt}}{V_{opt}\cdot\psi_{opt}}{W_{opt}\cdot\psi_{opt}^{-T}} =
\]
\[
\left \langle \begin{pmatrix*}[r] 0 & 1 & 0 & 1\\
0 & 0 & -1 & 1\\
0 & 1 & -1 & 1\\
1 & 0 & 0 & 0\\
0 & 1 & 0 & 0\\
-1 & 1 & -1 & 1\\
0 & 0 & 1 & 0
\end{pmatrix*},\,
\begin{pmatrix*}[r] 0 & 1 & 0 & 1\\
0 & 0 & -1 & 1\\
0 & 1 & -1 & 1\\
1 & 0 & 0 & 0\\
0 & 0 & 1 & 0\\
0 & 1 & 0 & 0\\
-1 & 1 & -1 & 1
\end{pmatrix*},\,
\begin{pmatrix*}[r] 0 & 0 & 1 & 1\\
0 & -1 & 0 & 1\\
0 & 1 & -1 & -1\\
1 & 0 & 0 & 0\\
1 & 1 & -1 & -1\\
0 & -1 & 0 & 0\\
0 & 0 & -1 & 0
\end{pmatrix*} \right \rangle
\]

It is easy to verify that $
\encdec{U_{opt}\cdot\psi_{opt}}{V_{opt}\cdot\psi_{opt}}{W_{opt}\cdot\psi_{opt}^{-T}} $
satisfy the triple product condition in Fact \ref{fact:Triple-product-condition}. Hence, they are encoding/decoding algorithm of an $\squarestrass{2}{7}$-algorithm. By Corollary \ref{cor:alt to mul}, the claim follows.
\end{proof}
\end{claim}

\begin{lemma}\label{lem:optbasis-flops}
Let $R$ be a ring, and let $A\in R^{n\times n}$ where $n=2^{k}$.
The arithmetic complexity of computing $\psi_{opt}\left(A\right)$ is 
$ F_{\psi_{opt}}\left(n\right)=n^{2}\log_{2}n $
The same holds for computing $\psi_{opt}^{-1}\left(A\right)$.
\begin{proof}
Both $\psi_{opt},\, \psi_{opt}^{-1}$ perform $q=4$ linear operations at each recursive step and has base case size of $n_{0}=2$. The lemma follows immediately from Lemma \ref{lem:basis runtime-1}.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lem:optbasis bw}Let $R$ be a ring, and let $A\in R^{n\times n}$ where $n=2^{k}$.
The I/O-complexity of computing $\psi_{opt}\left(A\right)$ is 
\[
IO_{\psi_{opt}}\left(n,M\right)\leq 2n^{2}\log_{2}\left(\sqrt{2}\frac{n}{\sqrt{M}}\right)+2M
\]
\begin{proof}
Both $\psi_{opt},\, \psi_{opt}^{-1}$ perform $q=4$ linear operations at each recursive step. The lemma follows immediately from Lemma \ref{lem:basis bw-1} with base case $n_{0}=2$.
\end{proof}
\end{lemma}

\begin{lemma}\label{lem:optaltRABS-flops} The arithmetic complexity of our $\squarestrass{2}{7}_{\psi_{opt}}$-algorithm is
$ F_{opt}\left(n\right)=5n^{\log_{2}7}-4n^{2} $
	\begin{proof}
Our $\squarestrass{2}{7}_{\psi_{opt}}$-algorithm has a $2\times 2$ base case and performs $7$ multiplications. Applying Fact \ref{rem:nnz} to its encoding/decoding matrices $\encdec{U_{opt}}{V_{opt}}{W_{opt}}$, we see that it performs 12 linear operations.
The result follows immediately from Lemma \ref{lem:RABS-flops}
	\end{proof}
\end{lemma}


\begin{lemma}
\label{lem:optalbilinearbw}The IO-complexity of our $\squarestrass{2}{7}_{\psi_{opt}}$-algorithm is
\begin{align*}
IO_{opt}\left(n,M\right) \leq & 12\cdot \left(\sqrt{3}\cdot M\left(\frac{n}{\sqrt{M}}\right)^{\log_{2} 7}-3n^{2}\right)+ \\
& +3M 
\end{align*}
\begin{proof}
Our algorithm has a $2\times 2$ base case and performs $7$ multiplications. By applying Fact \ref{rem:nnz} to its encoding/decoding matrices (as shown in Figure \ref{fig:optstrass}), we see that it performs 12 linear operations.
The result follows immediately from Lemma \ref{lem:bilinear bw-1}.
\end{proof}
\end{lemma}

\begin{corollary}
The computational complexity of {\em ABS} (Algorithm \ref{alg:ABS}) with our $\squarestrass{2}{7}_{\psi_{opt}}$ is
\begin{align*}
F_{ABS}\left(n\right)&= 5n^{\log_{2}7}-4n^{2} + 3n^2\log_{2}n
\end{align*}
	\begin{proof}
	The proof is similar to that of Corollary \ref{cor:absflops}
	\end{proof}
\end{corollary}

\begin{corollary}
Let $\bmapss:R^{n_{0}\times n_{0}}\to R^{n_{0}\times n_{0}}$
be invertible linear maps, and let {\em ALG} be an \\ $\squarestrassaltdef{n_{0}}{t}{}$-algorithm which performs $q$ linear operations at the base case.
The IO-complexity of {\em ABS} (Algorithm \ref{alg:ABS}) is
	\begin{align*}
	  IO_{ALG}\left(n,M\right) \leq & \left(\frac{3q}{t-n_{0}^{2}}\right)\left(M\left(\frac{\sqrt{3}\cdot n}{\sqrt{M}}\right)^{\omega_{0}}-n^{2}\right) + \\
	  & +3M + O\left(n^2\log \frac{n}{\sqrt{M}} \right)	
	\end{align*}
	\begin{proof}
The proof is similar to that of Corollary \ref{cor:absbw}
	\end{proof}

\end{corollary}

\begin{claim}
\label{lem:bilinear ks} Our $\squarestrass{2}{7}_{\psi_{opt}}$-algorithm's sequential and parallel IO-complexity is bound by $\Omega \left(\left(\frac{n}{\sqrt{M}}\right)^{\omega_{0}}M\right)$ and $\Omega \left(\left(\frac{n}{\sqrt{M}}\right)^{\omega_{0}}\frac{M}{P}\right)$, respectively (where $P$ is the number of processors and $\omega_{0} = \log_{2}7$).
\begin{proof}
We refer to the undirected bipartite graph defined by the decoding matrix of our a Strassen-like algorithm as its decoding graph (i.e., the edge $\left(i,\,j\right)$ exists if $W_{i,j}\neq 0$). In \cite{ballard2012graph}, Ballard et al. proved that for any square recursive-bilinear Strassen-like algorithm with $n_{0} \times n_{0}$ base case which performs $t$ multiplications, if the decoding graph is connected then these bounds apply with $\omega_{0} = \log_{n_{0}}t$.

The decoding graph of our algorithm is connected. Hence, the claim is true.
\begin{comment}
drawing
\end{comment}

	\end{proof}
\end{claim}

\subsubsection{Basis-invariant lower bound on additions for $2\times 2$ matrix multiplication} \label{subsubsec: optbound}

In this section we prove Theorem \ref{thm:bound} which says that 12 additions
are necessary to compute $2\times2$ matrix multiplication recursively
with base case of $2\times2$ and 7 multiplications, irrespective
of basis. Theorem \ref{thm:bound} completes Probert's lower bound which says that
for standard basis, 15 additions are required.

\begin{definition}
We denote the permutation matrix which swaps row-order for column-order
of vectorization of an $I\times J$ matrix by $P_{I\times J}$.
\end{definition}
\begin{lemma}
\label{lem:hop-perm}\cite{hopcroft1973duality} Let $\encdec{U}{V}{W}$
be the encoding/decoding matrices of an $\strass{m}{k}{n}{t}$-algorithm. Then $
\left\langle WP_{n\times m},\,U,\,VP_{n\times k}\right\rangle $
are encoding/decoding matrices of an $\left\langle n,m,k;t\right\rangle $-algorithm.
\end{lemma}

We use the following results, shown by Hopcroft and Kerr \cite{hopcroft1971minimizing}:
\begin{lemma}
\label{lem:-hopker1}\cite{hopcroft1971minimizing} If an algorithm
for $2\times2$ matrix multiplication has $k$ left (right) hand side multiplicands
of forms $A_{1,1},\,\left(A_{1,2}+A_{2,1}\right)$ and $\left(A_{1,1}+A_{1,2}+A_{2,1}\right)$, where additions are done modulu 2 then it requires at least $6+k$
multiplications
\end{lemma}
\begin{corollary}
\cite{hopcroft1971minimizing} \myworries{Similar results as to Lemma} \ref{lem:-hopker1}
apply for:
\begin{enumerate}
\item $\left(A_{1,1}+A_{2,1}\right),\left(A_{1,2}+A_{2,1}+A_{2,2}\right),\,\left(A_{1,1}+A_{1,2}+A_{2,2}\right)$
\item $\left(A_{1,1}+A_{1,2}\right),\left(A_{1,2}+A_{2,1}+A_{2,2}\right),\,\left(A_{1,1}+A_{2,1}+A_{2,2}\right)$
\item $\left(A_{1,1}+A_{1,2}+A_{2,1}+A_{2,2}\right),\left(A_{1,2}+A_{2,1}\right),\, \left(A_{1,1}+A_{2,2}\right)$
\item $A_{2,1},\left(A_{1,1}+A_{2,2}\right),\left(A_{1,1}+A_{2,1}+A_{2,2}\right)$
\item $\left(A_{2,1}+A_{2,2}\right),\left(A_{1,1}+A_{1,2}+A_{2,2}\right),\, \left(A_{1,1}+A_{1,2}+A_{2,1}\right)$
\item $A_{1,2},\left(A_{1,1}+A_{2,2}\right),\left(A_{1,1}+A_{1,2}+A_{2,2}\right)$
\item $\left(A_{1,2}+A_{2,2}\right),\left(A_{1,1}+A_{2,1}+A_{2,2}\right),\, \left(A_{1,1}+A_{1,2}+A_{2,1}\right)$
\item $A_{2,2},\left(A_{1,2}+A_{2,1}\right),\left(A_{1,2}+A_{2,1}+A_{2,2}\right)$
\end{enumerate}
\end{corollary}

%\begin{lemma}\cite{hopcroft1971minimizing} Any algorithm for $2\times2$ matrix multiplication which has $k$ left hand multiplicands of type $A_{1,1},\,A_{1,2},\,\left(A_{1,1}+A_{1,2}\right)$ ,where additions are modulu 2, requires at least $\left\lceil 6+\frac{k}{2}\right\rceil $ multiplications
%\end{lemma}

%\begin{lemma}\cite{hopcroft1971minimizing} Any algorithm for $2\times2$ matrix multiplication which has $k$ left hand multiplicands of type $A_{2,1},\,A_{2,2},\,\left(A_{2,1}+A_{2,2}\right)$ (where additions are modulu 2) requires at least $\left\lceil 6+\frac{k}{2}\right\rceil $ multiplications
%\end{lemma}

\begin{corollary}
\label{cor:Hop Kerr}Any $2\times2$ matrix multiplication algorithm
where a left hand (or right hand) multiplicand appears at least twice (modulu 2)
requires $8$ or more multiplications.
\end{corollary}

\begin{fact}
\label{fact:counting}A simple counting argument shows that any $7\times4$
binary matrix with less than 10 non-zero entries has a duplicate row
(modulu 2) or a zeroed out row.
\end{fact}

\begin{lemma}
\label{lem:Irrespective-of-basis-enc}Irrespective of basis transformations
$\phi,\,\psi$, $\upsilon$, the encoding matrices $U,\,V$, of a $\squarestrassaltdef{2}{7}$-algorithm
have no duplicate rows.
\begin{proof}
Let $\encdec{U}{V}{W} $ be encoding/decoding matrices
of an $\squarestrassaltdef{2}{7}$-algorithm. By Corollary
\ref{cor:alt to mul}, $\encdec{U\phi}{V\psi}{W\upsilon^{-T}}$
are encoding/decoding matrices of a $\squarestrass{2}{7}$-algorithm.
Assume, w.l.o.g, that $U$ contains a duplicate row, which means that
$U\phi$ contains a duplicate row as well. In that case, $\encdec{U\psi}{V\psi}{W\upsilon^{-T}}$
is a $\squarestrass{2}{7}$-algorithm in which one of the encoding matrices contains a duplicate
row, in contradiction to Corollary \ref{cor:Hop Kerr}.
\end{proof}
\end{lemma}

\begin{lemma}
\label{lem:encodingsparsity}Irrespective of basis transformations $\bmapss$, the encoding matrices $U,V$, of a $\squarestrassaltdef{2}{7}$-algorithm have at least $10$ non-zero entries.
\begin{proof}
Now row in $U,V$ can be zeroed out since otherwise the algorithm would require less than 7 multiplications. The result then follows from Fact \ref{fact:counting} and Lemma \ref{lem:Irrespective-of-basis-enc}.
\end{proof}
\end{lemma}
%
\begin{lemma}
\label{lem:decodingsparsity}Irrespective of basis transformations
$\phi, \, \psi$, $\upsilon$, the decoding matrix $W$ of an $\squarestrassaltdef{2}{7}$-algorithm
has at least $10$ non-zero entries.
\begin{proof}
Let $\left\langle U,V,W\right\rangle $ be encoding/decoding matrices
of an \\ $\squarestrassaltdef{2}{7}$-algorithm and suppose
by contradiction that $W$ has less than 10 non-zero entries. $W$
is a $7\times4$ matrix and so, by Fact \ref{fact:counting} states
that it either has a duplicate row (modulu 2) or a zeroed out row.
Corollary \ref{cor:alt to mul} states that $\left\langle U\phi,V\psi,W\upsilon^{-T}\right\rangle $
are encoding/decoding matrices of a $\left\langle 2,2,2;7\right\rangle $-algorithm.
Lemma \ref{lem:hop-perm} states that because $\left\langle U\phi,V\psi,W\upsilon^{-T}\right\rangle$ define a $\left\langle 2,2,2;7\right\rangle $-algorithm, so does
$\left\langle W\upsilon^{-T}P_{2\times2},U\phi,V\psi P_{2\times2}\right\rangle $.
Hence $W\upsilon^{-T}P_{2\times2}$ is an encoding matrix of a $\left\langle 2,2,2;7\right\rangle $-algorithm
which has duplicate or zeroed out rows, contradicting Corollary \ref{cor:Hop Kerr}.
\end{proof}
\end{lemma}

\begin{proof}[Proof (of Theorem \ref{thm:bound})]
Lemma \ref{lem:encodingsparsity}
and \ref{lem:decodingsparsity} then show that each encoding/decoding
matrix must contain at least 10 non-zero entries. By Remark \ref{rem:nnz}, the number of additions used by each of the encoding
matrix is $\nnz{U}-rows\left(U\right)$ (and analogously for $V$) and the
number of additions used by the decoding is $\nnz{W}-cols\left(W\right)$.
Hence, 12 additions are necessary for an $\squarestrassaltdef{2}{7}$-algorithm
irrespective of basis transformations $\bmapss$.
\end{proof}

%We have shown that our $\squarestrass{2}{7}_{\psi_{opt}}$, as defined in Figure \ref{fig:optstrass} and Notation \ref{notation:optbase},  performs 12 additions. Hence, by our lower bound in Theorem \ref{thm:bound}, it is optimal.
